Nonparametric Regression in Nonstandard Spaces

A nonparametric regression setting is considered with a real-valued covariate and responses from a metric space. One may approach this setting via Fr\'echet regression, where the value of the regression function at each point is estimated via a Fr\'echet mean calculated from an estimated objective function. A second approach is geodesic regression, which builds upon fitting geodesics to observations by a least squares method. These approaches are applied to transform two of the most important nonparametric regression estimators in statistics to the metric setting -- the local linear regression estimator and the orthogonal series projection estimator. The resulting procedures consist of known estimators as well as new methods. We investigate their rates of convergence in a general setting and compare their performance in a simulation study on the sphere.

==> discussion.tex <==
\section{Discussion}\label{sec:dicuss}
%
In this section, we want to critically discuss the results presented in this article  and their assumptions.

\subsection{\textsc{Entropy}}

The condition \textsc{Entropy} is a requirement for all error bounds above. It is fulfilled in many spaces, but it also excludes some, e.g., infinite dimensional Banach spaces. It can be an obstacle in the search of an interesting example of non-Euclidean and unbounded Hadamard space: In the model space of constant negative curvature $-1$, the hyperbolic plane $\mb H^2$, balls of radius $r>0$ have area $4\pi\sinh(r)^2$. Thus, for the covering number of a ball with radius $R>2$,
\begin{align*}
	\log\brOf{N(\ball(o, d_{\mb H^2}, R), d_{\mb H^2}, r)} 
	\geq 
	2\log\brOf{\frac{\sinh(R)}{\sinh(r)}} 
	\geq	
	2(R - r - 1)
	\eqcm
\end{align*}
so that
\begin{equation*}
\int_0^\infty \sqrt{\log\brOf{N(\ball(o, d_{\mb H^2}, R), d_{\mb H^2}, r)} } \dl r
\geq c\int_0^{R-1} \sqrt{R - r - 1}\, \dl r = c R^{\frac32}
\eqfs
\end{equation*}
Even so $\gamma_2(\ball(o, d_{\mb H^2}, R), d_{\mb H^2})$  might be smaller, it does not seem plausible to obtain the required bound.
Similarly, metric trees of infinite diameter and infinite branches do not seem to fulfill \textsc{Entropy}. 

To deal with spaces in which a ball of radius $R\geq1$ has an entropy integral of order $R^\alpha$, $\alpha>1$, one can replace the bound $\gamma_2(\mc B, d) \leq C_{\ms{Ent}} \diam(\mc B, d)$ required in \textsc{Entropy} by $\gamma_2(\mc B, d) \leq C_{\ms{Ent}} \max(\diam(\mc B, d), \diam(\mc B, d)^\alpha)$ for an $\alpha \in [1,2)$ and require a moment bound in \textsc{Moment} of order $\kappa  > \frac2{2-\alpha}$. This will yield the same rate of convergence. Further weakening of \textsc{Entropy} is possible, see \cite{ahidar20} and \cite{schoetz19}, potentially at the cost of a worse rate of convergence.

Note that the Hadamard spaces of trees with a fixed finite maximum number of branches do fulfill the  \textsc{Entropy} condition of the previous sections as they can be represented as a finitely many convex subsets of Euclidean spaces glued together \cite{billera01}.

\subsection{\textsc{ExpMap}}

\textsc{ExpMap} or (its generalization \textsc{IntBoundsSup} in the supplement) are not fulfilled for branching geodesics, i.e., if there are geodesics $\gamma_1, \gamma_2$ such that $\gamma_1(t) = \gamma_2(t)$ for $t \in [a,b]$ for $a<b$ and  $\gamma_1(t) \neq \gamma_2(t)$ for $t \in [a\pr,b\pr]$ for $a\pr<b\pr$. The reason is that in this case the integral over the distance of the geodesics on an interval can be of smaller order that the supremum of the distance of the two geodesics on the interval. Similarly, if the distance between two geodesics increases two quickly (like in the hyperbolic plane), \textsc{ExpMap} might also not be fulfilled.

\subsection{Smoothness}

\texttt{LocFre} and \texttt{OrtFre} do not require \textsc{ExpMap}. But their smoothness condition is not fully satisfactory. The roughness of the change of the error density should not be that important, given that the regression function changes smoothly. It is likely an artifact of the proof that we require the error density to be smooth. 

\subsection{Gaussian Concentration}

In bounded space, it might be possible to improve the results to obtain not only bounds in expectation but also Gaussian concentration by following \cite{ahidar20} and making use of \textit{Talagrand's inequality} \cite{bousquet02}.
%
